Rethinking the Roles of Diffusion and Decoding: Predictive-State Flows for Parallel Language Generation

In continuous diffusion language models (DLMs), latents generated by the diffusion prior are mapped almost deterministically to tokens, either by a decoder or through a token embedding matrix. Unlike in image generation, where visual details can vary continuously, the diffusion prior must capture fine-grained discrete token choices in continuous space, which can make the joint latent distribution difficult to model. We argue that generative roles should instead be divided: the diffusion prior should generate high-level predictive information, while the decoder should resolve the remaining token-level choices. Based on this view, we introduce Predictive-State Flows (PSF), which partitions a sequence into blocks and associates each block with a predictive state computed solely from the preceding context. A rectified-flow prior generates the sequence of predictive states, after which a block-causal decoder generates all blocks in parallel, autoregressively only within each block. This design reduces diffusion from L token-level states to K << L predictive states and reduces token-level sequential depth to L/K. On unconditional OpenWebText generation, a 197M-parameter model with K=8 achieves a generative perplexity of 22.8 at entropy 5.16 using 0.31 TFLOPs per 1024-token document, versus 24.0 and 7.2 TFLOPs for ELF-B with 32 sampling steps. The corresponding measured operating points yield MAUVE@512 of 0.93 and 0.73, respectively. Controlled comparisons further show that content states, which additionally encode their own blocks, yield 8-16% higher generative perplexity than predictive states, and that replacing sampled predictive-state trajectories with a shared mean lowers MAUVE@512 by 0.11. These results suggest that latent design for continuous DLMs should consider not only how compactly text is represented, but also how generative roles are divided between the prior and the decoder.

==> fig_architecture_style.tex <==
% Shared drawing styles for the three appendix diagrams, split from the former Figure 1.
\colorlet{ovBlue}{black!60}%
\colorlet{ovGreen}{black!60}%
\colorlet{ovGold}{black!60}%
\colorlet{ovPurple}{black!60}%
\colorlet{ovLine}{black!65}%
\colorlet{ovInk}{black}%
\colorlet{ovFlow}{black!65}%
\colorlet{ovDecoder}{black!65}%
\colorlet{ovDecoderFill}{white}%
\begin{tikzpicture}[
  x=1cm,y=-1cm,text=ovInk,
  font=\fontsize{12}{13.5}\selectfont,
  every node/.style={inner sep=0pt,outer sep=0pt},
  head/.style={font=\fontsize{12.5}{14}\selectfont,align=center},
  sub/.style={font=\fontsize{11.7}{13.5}\selectfont,align=center},
  labeltext/.style={font=\fontsize{11.5}{13}\selectfont,align=center},
  state/.style={draw=black!65,fill=black!8,
    rounded corners=.5pt,line width=.5pt,
    minimum width=.88cm,minimum height=.53cm,
    font=\fontsize{13}{14}\selectfont},
  token/.style={draw=black!65,fill=white,
    rounded corners=.5pt,line width=.5pt,minimum height=.43cm,
    minimum width=.88cm,font=\fontsize{10.7}{12}\selectfont},
  prefixblock/.style={draw=ovBlue,fill=white,rounded corners=.5pt,
    line width=.5pt,minimum width=.62cm,minimum height=.40cm,
    font=\fontsize{10.7}{12}\selectfont},
  arr/.style={-{Latex[length=1.8mm,width=1.15mm]},draw=ovLine,line width=.65pt},
  brace/.style={draw=ovLine,line width=.65pt},
  landing/.style={-{Latex[length=2.0mm,width=1.3mm]},draw=ovFlow!80!black,
    line width=.9pt,dash pattern=on 3pt off 1.7pt},
  decoder/.style={draw=ovDecoder,fill=ovDecoderFill,rounded corners=1pt,
    line width=.65pt,minimum width=2.05cm,minimum height=.56cm,
    font=\fontsize{10.7}{12}\selectfont}
]

